What is a Social Media Bot? A Global Comparison of Bot and Human Characteristics

Chatter on social media is 20% bots and 80% humans. Chatter by bots and humans is consistently different: bots tend to use linguistic cues that can be easily automated while humans use cues that require dialogue understanding. Bots use words that match the identities they choose to present, while humans may send messages that are not related to the identities they present. Bots and humans differ in their communication structure: sampled bots have a star interaction structure, while sampled humans have a hierarchical structure. These conclusions are based on a large-scale analysis of social media tweets across ~200mil users across 7 events. Social media bots took the world by storm when social-cybersecurity researchers realized that social media users not only consisted of humans but also of artificial agents called bots. These bots wreck havoc online by spreading disinformation and manipulating narratives. Most research on bots are based on special-purposed definitions, mostly predicated on the event studied. This article first begins by asking, "What is a bot?", and we study the underlying principles of how bots are different from humans. We develop a first-principle definition of a social media bot. With this definition as a premise, we systematically compare characteristics between bots and humans across global events, and reflect on how the software-programmed bot is an Artificial Intelligent algorithm, and its potential for evolution as technology advances. Based on our results, we provide recommendations for the use and regulation of bots. Finally, we discuss open challenges and future directions: Detect, to systematically identify these automated and potentially evolving bots; Differentiate, to evaluate the goodness of the bot in terms of their content postings and relationship interactions; Disrupt, to moderate the impact of malicious bots.

==> socialmediaplatforms.tex <==
\section{Social Media Platforms}
\todo{user, content, interactions}

Here we expound on the ``technical" portion of our ``socio-technical" portion. The activity of social media bots take place on social media platforms, which provides the technical information infrastructure for social interactions to take place, sometimes facilitating these interactions. The social media platform is a complex ecosystem that essentially consists of three main elements: \textbf{users, content and relationships} \cite{howard2012social}. Users are represented by their virtual accounts, are the key actors driving the system, creating and distributing information. Content is the information generated by users on the platform. Relationships are formed from the user-user, user-content and content-content interactions. As of April 2024, the most commonly used social media platforms are: Facebook, X, Instagram, TikTok \cite{statistaBiggestSocial}.

\paragraph{User} There are three types of social media users: the account, the operator and the agents. An \textit{account} is the digital persona of a user, the online identity that the user discloses through his posts and interactions on the platform. The \textit{operator} is the human person who controls the account: for humans, the operator is usually the human himself, while for automated bot accounts, the operator is usually controlling more than one account. The  An \textit{agents} is an actively contribution user, whose actions affect the other users on the platform. All accounts are users, but only a few of them are agents.

\paragraph{Content} Content are articles and information generated by Users. The type of Content ranges from text to image to video, and are dependent on the storytelling media available on the platform. Content forms the basis where users tell their stories and receive updates from other users.

\paragraph{Interactions} Interactions refer to the communication and actions between people, or between users in the social media world. The social media platform is a medium for user interactions to occur, and sometimes facilitate these interactions. There are two main types of interactions: \textit{Communication Interactions}, which are performed using interaction mechanics such as sharing a post or tagging another user. \textit{Relationship interactions} are performed through network building mechanic such as following another user. 

\todo{Social media primitives diagram?}

\todo{this section doesn't really link with the rest...}
